Efficient Arbitrary Precision Acceleration for Large Language Models on GPU Tensor Cores

Large language models (LLMs) have been widely applied but face challenges in efficient inference. While quantization methods reduce computational demands, ultra-low bit quantization with arbitrary precision is hindered by limited GPU Tensor Core support and inefficient memory management, leading to suboptimal acceleration. To address these challenges, we propose a comprehensive acceleration scheme for arbitrary precision LLMs. At its core, we introduce a novel bipolar-INT data format that facilitates parallel computing and supports symmetric quantization, effectively reducing data redundancy. Building on this, we implement an arbitrary precision matrix multiplication scheme that decomposes and recovers matrices at the bit level, enabling flexible precision while maximizing GPU Tensor Core utilization. Furthermore, we develop an efficient matrix preprocessing method that optimizes data layout for subsequent computations. Finally, we design a data recovery-oriented memory management system that strategically utilizes fast shared memory, significantly enhancing kernel execution speed and minimizing memory access latency. Experimental results demonstrate our approach's effectiveness, with up to 2.4\times speedup in matrix multiplication compared to NVIDIA's CUTLASS. When integrated into LLMs, we achieve up to 6.7\times inference acceleration. These improvements significantly enhance LLM inference efficiency, enabling broader and more responsive applications of LLMs.

==> chapters/3_design1_origin.tex <==
\section{ARBITRARY PRECISION MATMUL}\label{APMM}
% The most time-consuming operation in Transformer model inference is matrix multiplication (MatMul). Additionally, the redundancy caused by unsupported data formats is primarily reflected in matrix multiplication. Therefore, the key objective of this paper is to implement arbitrary precision matrix multiplication during model inference. 

In this section, we implement MatMul for arbitrary precision INT data using TCs. First, we decompose the input data bit by bit, breaking down arbitrary precision data into 1-bit data which is supported by TCs for MatMul, and design the corresponding data flow abstraction. Next, we introduce a bipolar-INT data format to replace the original INT format for MatMul and analyze the advantages of this approach.

%\subsection{Bit-Wise MatMul Decomposition}\label{subsec:Decomposition}
\subsection{Decomposition-Based MatMul}\label{subsec:Decomposition}
Assume an arbitrary precision \msb{MatMul} operation involves matrix $W$ with $n_w$ bits and matrix $X$ with $n_x$ bits, ultimately calculating a 32-bit output $Y=WX$. An n-bit data can be decomposed into n 1-bit data, and it is equivalent to the sum of these data shifted accordingly. So we first decompose $W$ and $X$ bit by bit into $n_w$ and $n_x$ matrices, denoted as $W^{(i)}$ and $X^{(j)}$
% For example, a 3-bit data $a$ can be decomposed into three 1-bit data:
% \[a:a^{(2)}a^{(1)}a^{(0)}~with~a^{(i)}\in int1\]
% \[a^{(i)}=(a\gg i)\&1,~~a=\sum_{i=0}^2a^{(i)}\ll i\]

% Therefore, for the multiplication of any two numbers $w*x$ from matrices $W$ and $X$:
% \begin{equation}
%     w=\sum_{i=0}^{n_w-1}w^{(i)}\ll i,~x=\sum_{j=0}^{n_x-1}x^{(j)}\ll j
% \end{equation}

% Using the 1-bit operation $OP(a,b)$, which takes a 1-bit input and produces a 32-bit output.
% \begin{equation}
%     wx=\sum_{i=0}^{n_w-1}\sum_{j=0}^{n_x-1}OP(w^{(i)},x^{(j)})\ll (i+j)
% \end{equation}

\msb{After the data decomposition, we use \msb{TC}s to perform \msb{MatMul} on the 1-bit matrices of $W$ and $X$ pairwise, resulting in a 32-bit intermediate result matrix $Y^{(i,j)}$. After the Ampere architecture, Nvidia GPUs support the selection of either AND or XOR logic for 1-bit MatMul operations within Tensor Cores}

% When invoking \msb{TC}s for 1-bit data computation, the operation is not limited to single data elements but rather applies to entire matrices. Therefore, we first need to decompose each n-bit data element in the matrix and concatenate the same bit positions to obtain n 1-bit matrices. Then, we use \msb{TC}s to perform \msb{MatMul} on the 1-bit matrices of $W$ and $X$ pairwise, resulting in a 32-bit intermediate result matrix $Y^{(i,j)}$. 
Finally, we shift and add the intermediate result matrices based on their bit $(i,j)$ to recover the final output. The complete computation process of arbitrary precision matmul is illustrated in Fig. \ref{fig:AP-bit-matmul}.
% \begin{equation}
%     Y^{(i,j)}=W^{(i)}X^{(j)}
% \end{equation}
% \begin{equation}
%     Y=\sum_{i=0}^{n_w-1}\sum_{j=0}^{n_x-1}Y^{(i,j)}\ll (i+j)
% \end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/APBit MatMul.png}
    \caption{Illustration of the computation process of arbitrary precision MatMul. Here matrices W and X are both 2-bit, a can be extended to arbitrary bit widths.}
    \label{fig:AP-bit-matmul}
\end{figure}

\subsection{Bipolar-INT Data Format}
We propose a novel \msb{data format called bipolar-INT, which is suitable for symmetric quantization and conducive to parallel computation,} for data quantization and \msb{MatMul}. Specifically, in typical INT data, each bit takes a value of 0 or 1, while in bipolar-INT data, a "0" is considered as "-1" during computation, meaning each bit can take on values of -1 or 1. 
% For a 2-bit example, the comparison of different data formats is shown in the TABLE \ref{tab:my_label} below. It is evident that bipolar-INT can represent odd numbers within a symmetric range. 

% During \msb{MatMul}, it is only necessary to change the multiplication operation from the "AND" operation to the "XOR" operation, which is also supported by the \msb{TC}.


% \begin{table}[h]
%     \centering
%     \begin{tabular}{c||c|c|c}
%         \hline
%         Binary Format & Unsigned INT & Signed INT & bipolar-INT\\
%         \hline
%         00 & 0 & 0 & -3\\
%         \hline
%         01 & 1 & 1 & -1\\
%         \hline
%         10 & 2 & -2 & 1\\
%         \hline
%         11 & 3 & -1 & 3\\
%         \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

% In the following text, we will analyze in detail the advantages of bipolar-INT in model quantization and \msb{MatMul}.

\subsubsection{Bipolar-INT in Model Quantization}
    
The advantage of bipolar-INT in quantization lies in its inherently zero-centered symmetric representation, which eliminates the need for additional zero-point offset matrices and avoids the need for special sign bits and two's complement arithmetic.

For signed INT quantization, due to the presence of two's complement arithmetic, the sign of the MSB matrix after decomposition is opposite to the signs of the other bits. This requires separate handling during subsequent \msb{MatMul} and matrix reconstruction, which is highly unfavorable for the parallel computation of single-bit matrices at each bit (Fig. \ref{fig:bipolar compare}).    

For unsigned INT quantization, the presence of an additional zero-point offset introduces extra multiply-accumulate operations during \msb{MatMul}, which is also detrimental to the optimization of matrix multiplication (Fig. \ref{fig:bipolar compare}).
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/bipolar and original 2.png}
    \caption{Compared to original signed and unsigned integers, bipolar-INT is suitable for parallel computing and symmetric quantization.}
    \label{fig:bipolar compare}
\end{figure}

% \begin{equation}
%     WX=\hat W\hat X+Z_x\hat W+ Z_w\hat X+Z_wZ_x
% \end{equation}
    


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/bipolar与int对比.png}
%     \caption{
% Compared to signed integers, bipolar-INT does not have special sign bits, which makes it more conducive to parallel computing.}
%     \label{fig:bipolar int}
% \end{figure}
    
% \begin{equation}
% \begin{split}
%     WX=\sum_{\substack{i\neq n-1\\j\neq n-1}}W^{(i)}X^{(j)}-\sum_{\substack{i=n-1\\j\neq n-1}}W^{(i)}X^{(j)}\\
%     -\sum_{\substack{i\neq n-1\\j=n-1}}W^{(i)}X^{(j)}+W^{(n-1)}X^{(n-1)}
% \end{split}
% \end{equation}
    
\subsubsection{Bipolar-INT in \msb{MatMul}}

The advantage of bipolar-INT in \msb{MatMul} lies in its compatibility with the quantization method of binary neural networks, eliminating the need for additional operations during \msb{MatMul} and thereby saving substantial overhead.
    
\msb{For neural networks employing binary quantization, weights are often quantized into two values: (-1, 1). 
For our work, this quantization method is highly compatible with bipolar-INT. By quantizing the feature matrix into the bipolar-INT format, we can directly use standard bipolar-INT matrix multiplication operations.}

\msb{However, if the feature matrix is quantized using traditional INT quantization, for example, compute the MatMul of $W=[-1,1]$ and $X=[1,0]$. The method proposed by APNN-TC\cite{apnn-tc} introduces an additional all-ones matrix $J=[1,1]$. When read as an int type, the matrix X is read as $\hat{W}=[0,1]$, which relates to the actual data by $W=2\hat{W}-J$. Thus, the MatMul becomes $WX=2\hat{W}X-JX$.}

% the single-bit multiplication might produce three values (-1, 0, 1), which cannot be represented by a single bit. In the APNN paper\cite{apnn-tc}, a matrix $J$ with values of 1 was introduced for computation, resulting in additional storage and computational overhead.

% \begin{equation}
%     \hat W=\frac{W+J}{2}
% \end{equation}
% \begin{equation}
%     WX=2\hat WX-JX
% \end{equation}


% The W matrix has bit values of -1/1. By applying the transformation described in equation 7, these bit values can be converted to 0/1. Incorporating this transformation into matrix multiplication results in equation 8.

==> chapters/4_design2_origin.tex <==
\section{GPU MEMORY SCHEDULING}
% The GPU is composed of a multi-level memory hierarchy, with different memory levels varying in size and processing speed. Global memory, accessible by all threads, has the largest size but the slowest processing speed. In contrast, shared memory is only accessible by threads within a block, has much smaller size but much faster processing speed compared to global memory. Specifically, to match the processing speed of Tensor Cores, the GPU includes a set of extremely fast registers called fragments, which are dedicated to storing the inputs, outputs, and intermediate results of Tensor Core operations.

This section focuses on how to efficiently transfer data between different levels of the memory hierarchy in the arbitrary precision \msb{MatMul} kernel to maximize processing speed. 
% The complete GPU multi-level memory scheduling scheme is illustrated in Fig. \ref{fig:GPU-Mem-Scheduling}. 

\subsection{Matrix Decomposition and Reassembly}

On one hand, similar to how \msb{TC} data formats do not support all INT precisions, GPUs support more precisions than \msb{TC}s when accessing memory, but still do not support all possible precisions \msb{(Step 0 in Fig. \ref{fig:decomposition and reassembly})}.
% For example, a 3-bit INT type does not have a suitable storage format, so it must be stored using a wider data format (such as 4-bit or 8-bit), which clearly introduces redundant memory access overhead.

On the other hand, when the amount of data we need to access is large, we not only need to consider whether the storage precision is supported but also whether the corresponding data format is conducive to data transfer. For instance, CPUs and GPUs have native support for 32-bit data types, which includes benefits such as data alignment, memory access efficiency, and optimized processor instruction sets. These factors all influence data transfer speed. However, 4-bit or 8-bit data types do not enjoy such support.
% Consequently, when transmitting the same amount of data, encapsulating it into a 32-bit data format is more conducive to faster data transfer. 
% For example, storing 64 4-bit data elements in 8 INT\msb{32}s is more efficient for data transfer.

Therefore, we need to preprocess the original $n$-bit INT matrix \msb{to reduce memory access redundancy and transmit data more efficiently}. First, we perform single-bit decomposition on the original matrix, breaking down each bit and regrouping them with corresponding bits from other data to form $n$ single-bit matrices \msb{ (Step 1 in Fig. \ref{fig:decomposition and reassembly})}. This step circumvents the issue of unsuitable data formats and eliminates memory redundancy caused by the lack of appropriate data formats. Next, we \msb{reassemble} the decomposed data using 32-bit unsigned INTs \msb{ (Step 2 in Fig. \ref{fig:decomposition and reassembly})}. This step ensures that the input data aligns with the GPU's native support, thereby enhancing data transfer speed. Finally, we sequentially concatenate the processed $n$ matrices into a single matrix \msb{(Step 3 in Fig. \ref{fig:decomposition and reassembly})}. This step not only further conserves memory but also simplifies $n$ data transfer instructions into a single instruction. Although the amount of data transferred remains the same, this concatenation improves data transfer speed and saves storage space.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/decomposition and reassembly.png}
    \caption{GPU Shared Memory Scheduling Design}
    \label{fig:decomposition and reassembly}
\end{figure}

\subsection{Warp-Level Block Processing}\label{subsec:Warp-Level}
First, we partition the output matrix by dividing the original $M\times N$ output matrix into several $b_m\times b_n$ regions(Fig. \ref{fig:GPU-Shared-Mem}.) Each block is responsible for computing the output within one region. If the number of regions exceeds the number of available blocks, the blocks are reused in multiple cycles.
Since the input is decomposed into the form of a single-bit matrix in advance, the data that each thread block needs to process is $b_m$ row data of $n_w$ weight single-bit matrices and $b_n$ row data of $n_x$ feature single-bit matrices, which can be regarded as an $n_wb_m\times K$ single-bit matrix and an $n_xb_n\times K$ single-bit matrix.
The reason for using such a complex processing method instead of simply calculating single-bit matmul directly will be explained later in \ref{subsubsec:DR-in-SHMEM}.


Then, due to the insufficient size of shared memory, the dimension $K$ needs to be partitioned. Each time, the thread block only reads data from two matrices of size $n_{w,x}b_{m,n}\times b_k$, and the results of each computation are accumulated over $K/b_k$ iterations to produce the complete output value. We allocate two blocks of shared memory of the same size. While one block is responsible for computation, the other block reads the next set of data. They then alternate in this manner, effectively hiding the data transfer latency from global memory to shared memory. 

Next, under normal circumstances, we would pair the \(n_w\) weight tiles with the \(n_x\) feature tiles, performing \(n_w \times n_x\) single-bit \msb{MatMul}s of size \((b_m, b_n, b_k)\). Given that \((b_m, b_n, b_k)\) values are relatively small, such repeated calculations reduce data reuse and increase data read latency. However, we observe that by concatenating multiple single-bit matrices within each block and treating them as a single \(n_wb_m \times b_k\) matrix and an \(n_xb_n \times b_k\) matrix for \msb{MatMul}, we can effectively reduce the number of data reads, increase data reuse, and significantly enhance the performance advantages of the \msb{TC}.

Finally, since \msb{TC} computations need to be performed within warps, we need to further partition the data in shared memory to be processed by each warp within the block. These data partitions are read into fragments, and \msb{TC}s are invoked for computation. It is important to address data reuse: each read of the weight matrix should be used to compute with as many feature matrices as possible. This not only increases data reuse but also facilitates partial shift-and-add operations directly within the fragments (which will be discussed in detail in SubSec. \ref{subsec:Data Recovery}).

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/GPU-Mem-Scheduling.png}
    \caption{Complete GPU Multi-Level Memory Scheduling Design}
    \label{fig:GPU-Mem-Scheduling}
\end{figure}

\subsection{Efficient Data Recovery}\label{subsec:Data Recovery}
Reviewing the data flow abstraction in Sec. \ref{subsec:Decomposition}, we decompose the input matrix into several single-bit matrices, multiply them pairwise to obtain intermediate result matrices, and then shift and add these intermediate results to get the final output. 

Generally, designing GPU memory scheduling with this approach means that each GPU block is responsible for multiplying one pair of single-bit matrices and then shifting and adding the results to obtain the output. However, in this process, each block only produces the result of one pair of \msb{MatMul}s, which must be returned to global memory for shifting and adding. At this point, the results are already 32-bit data, and the global memory's processing speed is very slow. Consequently, matrix recovery becomes the bottleneck in the \msb{MatMul} operation, and this step's delay can even drag down the performance of the \msb{MatMul} computation.

Therefore, we propose an efficient data recovery design that utilizes the faster shared memory and fragments to complete the data recovery operations. The specific details are as follows:

\subsubsection{Data Recovery in Shared Memory}\label{subsubsec:DR-in-SHMEM}

First, we naturally consider performing the matrix recovery operations in the faster shared memory as much as possible, converting the recovered data into a format that can be directly output before sending it back to the global memory. However, if we follow the general approach mentioned above, where each block is only responsible for the multiplication of one pair of single-bit matrices, the shared memory will contain only one set of outputs, making it impossible to complete the matrix recovery.

Thus, we load tiles of the same position and size from each single-bit matrix into the block for computation, rather than just choosing a pair of single-bit matrix tiles. For example, when computing \msb{MatMul} with weights being 2-bit, a block does not only contain tiles of $W_0$ or $W_1$, but tiles of both $W_0$ and $W_1$ of the same position and size. While this reduces the tile size of each single-bit matrix loaded into the block, it ensures that each block has all the data needed to compute a single output. This allows the intermediate results to be shifted and added directly in shared memory, with the final result being returned to global memory. This also explains why we use such a complex matrix loading strategy in \ref{subsec:Warp-Level}.

\subsubsection{Data Recovery in Fragment}\label{subsubsec:DR-in-Frag}

In the previous section, to improve data reuse, we had fragments read one weight tile and as many feature tiles as possible. Suppose a fragment within the same warp contains the lowest bit weight tile $W^{(0)}$ and all 
$n_x$ bit feature tiles $X^{(j)}$. By performing \msb{MatMul} for the bit positions of the feature tiles, we obtain $n_x$ intermediate results $Y^{(0,j)}$, which are then shifted and added to get the intermediate result corresponding to $W^{(0)}$. Subsequently, in shared memory, we only need to shift and add the different bit positions of the weights to obtain the final output. This phased data recovery design reduces the data recovery operation in shared memory from two loops to one and utilizes the faster processing speed of fragments to complete part of the data recovery, effectively reducing the latency in the data recovery phase.






